Numerical simulations of the Tayler-Spruit dynamo in proto-magnetars

The Tayler-Spruit dynamo is one of the most promising mechanisms proposed to explain angular momentum transport during stellar evolution. Its development in proto-neutron stars spun-up by supernova fallback has also been put forward as a scenario to explain the formation of very magnetized neutron stars called magnetars. Using three-dimensional direct numerical simulations, we model the proto-neutron star interior as a stably stratified spherical Couette flow with the outer sphere that rotates faster than the inner one. We report the existence of two subcritical dynamo branches driven by the Tayler instability. They differ by their equatorial symmetry (dipolar or hemispherical) and the magnetic field scaling, which is in agreement with different theoretical predictions (by Fuller and Spruit, respectively). The magnetic dipole of the dipolar branch is found to reach intensities compatible with observational constraints on magnetars.

==> supp_mat <==
\begin{thebibliography}{}
\makeatletter
\relax
\def\mn@urlcharsother{\let\do\@makeother \do\$\do\&\do\#\do\^\do\_\do\%\do\~}
\def\mn@doi{\begingroup\mn@urlcharsother \@ifnextchar [ {\mn@doi@}
  {\mn@doi@[]}}
\def\mn@doi@[#1]#2{\def\@tempa{#1}\ifx\@tempa\@empty \href
  {http://dx.doi.org/#2} {doi:#2}\else \href {http://dx.doi.org/#2} {#1}\fi
  \endgroup}
\def\mn@eprint#1#2{\mn@eprint@#1:#2::\@nil}
\def\mn@eprint@arXiv#1{\href {http://arxiv.org/abs/#1} {{\tt arXiv:#1}}}
\def\mn@eprint@dblp#1{\href {http://dblp.uni-trier.de/rec/bibtex/#1.xml}
  {dblp:#1}}
\def\mn@eprint@#1:#2:#3:#4\@nil{\def\@tempa {#1}\def\@tempb {#2}\def\@tempc
  {#3}\ifx \@tempc \@empty \let \@tempc \@tempb \let \@tempb \@tempa \fi \ifx
  \@tempb \@empty \def\@tempb {arXiv}\fi \@ifundefined
  {mn@eprint@\@tempb}{\@tempb:\@tempc}{\expandafter \expandafter \csname
  mn@eprint@\@tempb\endcsname \expandafter{\@tempc}}}

\bibitem[\protect\citeauthoryear{{Aubert}, {Gastine}  \& {Fournier}}{{Aubert}
  et~al.}{2017}]{aubert2017}
{Aubert} J.,  {Gastine} T.,   {Fournier} A.,  2017, \mn@doi [Journal of Fluid
  Mechanics] {10.1017/jfm.2016.789}, 813, 558

\bibitem[\protect\citeauthoryear{{Barr{\`e}re}, {Guilet}, {Reboul-Salze},
  {Raynaud}  \& {Janka}}{{Barr{\`e}re} et~al.}{2022}]{barrere2022}
{Barr{\`e}re} P.,  {Guilet} J.,  {Reboul-Salze} A.,  {Raynaud} R.,   {Janka}
  H.~T.,  2022, \mn@doi [Astron. Astrophys.] {10.1051/0004-6361/202244172},
  668, A79

\bibitem[\protect\citeauthoryear{{Cutler} \& {Lindblom}}{{Cutler} \&
  {Lindblom}}{1987}]{cutler1987}
{Cutler} C.,  {Lindblom} L.,  1987, \mn@doi [Astrophys. J.] {10.1086/165052},
  314, 234

\bibitem[\protect\citeauthoryear{{Gastine} \& {Wicht}}{{Gastine} \&
  {Wicht}}{2012}]{gastine2012}
{Gastine} T.,  {Wicht} J.,  2012, \mn@doi [Icarus]
  {10.1016/j.icarus.2012.03.018}, 219, 428

\bibitem[\protect\citeauthoryear{{Goossens} \& {Tayler}}{{Goossens} \&
  {Tayler}}{1980}]{goossens1980b}
{Goossens} M.,  {Tayler} R.~J.,  1980, \mn@doi [\mnras]
  {10.1093/mnras/193.4.833}, 193, 833

\bibitem[\protect\citeauthoryear{{Guilet}, {M{\"u}ller}  \& {Janka}}{{Guilet}
  et~al.}{2015}]{guilet2015b}
{Guilet} J.,  {M{\"u}ller} E.,   {Janka} H.-T.,  2015, \mn@doi [\mnras]
  {10.1093/mnras/stu2550}, 447, 3992

\bibitem[\protect\citeauthoryear{{H{\"u}depohl}}{{H{\"u}depohl}}{2014}]{hudepohl2014}
{H{\"u}depohl} L.,  2014, PhD thesis, Technical University of Munich, Germany

\bibitem[\protect\citeauthoryear{{Kelly}}{{Kelly}}{1973}]{kelly1973}
{Kelly} D.~C.,  1973, \mn@doi [\apj] {10.1086/151898}, \href
  {https://ui.adsabs.harvard.edu/abs/1973ApJ...179..599K} {179, 599}

\bibitem[\protect\citeauthoryear{Lee}{Lee}{1950}]{lee1950}
Lee T.~D.,  1950, \mn@doi [The Astrophysical Journal] {10.1086/145306}, 111,
  625

\bibitem[\protect\citeauthoryear{{Schaeffer}}{{Schaeffer}}{2013}]{schaeffer2013}
{Schaeffer} N.,  2013, \mn@doi [Geochemistry, Geophysics, Geosystems]
  {10.1002/ggge.20071}, 14, 751

\bibitem[\protect\citeauthoryear{{Schwaiger}, {Gastine}  \&
  {Aubert}}{{Schwaiger} et~al.}{2019}]{schwaiger2019}
{Schwaiger} T.,  {Gastine} T.,   {Aubert} J.,  2019, \mn@doi [Geophysical
  Journal International] {10.1093/gji/ggz192}, 219, S101

\bibitem[\protect\citeauthoryear{{Tayler}}{{Tayler}}{1973}]{tayler1973}
{Tayler} R.~J.,  1973, \mn@doi [Mon. Not. Astron. R. Soc.] {10.1093/Mon. Not.
  Astron. R. Soc./161.4.365}, 161, 365

\bibitem[\protect\citeauthoryear{{Thompson} \& {Duncan}}{{Thompson} \&
  {Duncan}}{1993}]{thompson1993}
{Thompson} C.,  {Duncan} R.~C.,  1993, \mn@doi [Astrophys. J.]
  {10.1086/172580}, 408, 194

\bibitem[\protect\citeauthoryear{{Wicht}}{{Wicht}}{2002}]{wicht2002}
{Wicht} J.,  2002, \mn@doi [Physics of the Earth and Planetary Interiors]
  {10.1016/S0031-9201(02)00078-X}, 132, 281

\makeatother
\end{thebibliography}

